Automated Pupillary Light Reflex Test on a Portable Platform

In this paper, we introduce a portable eye imaging device denoted as lab-on-a-headset, which can automatically perform a swinging flashlight test. We utilized this device in a clinical study to obtain high-resolution recordings of eyes while they are exposed to a varying light stimuli. Half of the participants had relative afferent pupillary defect (RAPD) while the other half was a control group. In case of positive RAPD, patients pupils constrict less or do not constrict when light stimuli swings from the unaffected eye to the affected eye. To automatically diagnose RAPD, we propose an algorithm based on pupil localization, pupil size measurement, and pupil size comparison of right and left eye during the light reflex test. We validate the algorithmic performance over a dataset obtained from 22 subjects and show that proposed algorithm can achieve a sensitivity of 93.8% and a specificity of 87.5%.

==> fig_results.tex <==
\begin{figure*}[htbp!]
\begin{minipage}[b]{0.48\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/results/RAPD1_AUC.png}
  \vspace{0.01cm}
  \centerline{\footnotesize{(a)}}%\medskip
  \vspace{0.03 cm}
\end{minipage}
\vspace{0.1cm}
\begin{minipage}[b]{0.48\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/results/RAPD1_scatter.png}
  \vspace{0.01cm}
  \centerline{\footnotesize{(b)}}%\medskip
  \vspace{0.03 cm}
\end{minipage}

\begin{minipage}[b]{0.48\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/results/RAPD2_AUC.png}
  \vspace{0.01cm}
  \centerline{\footnotesize{(c)}}%\medskip
  \vspace{0.03 cm}
\end{minipage}
\vspace{0.1cm}
\begin{minipage}[b]{0.48\linewidth}
  \centering
\includegraphics[width=\textwidth]{./Figs/results/RAPD2_scatter.png}
  \vspace{0.01cm}
  \centerline{\footnotesize{(d)}}%\medskip
  \vspace{0.03 cm}
\end{minipage}

\centering
\vspace{-4 mm}
\caption{fig:results}
\end{figure*}

==> table_datasets.tex <==
\begin{table*}[htbp!]
\centering
\centering
\caption{Existing pupil datasets captured with closely-mounted setups and the RAPD-HD dataset.*}
\label{tab:datasets}
\begin{threeparttable}
\begin{tabular}{> {\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{1.4cm}>{\centering\arraybackslash}p{2.2cm}>{\centering\arraybackslash}p{2.5cm}}
\hline
\textbf{}  & 
\textbf{\href{https://www.cl.cam.ac.uk/research/rainbow/projects/pupiltracking/datasets/}{Swirski}~\cite{Swirski2012}}  & \textbf{Kasneci }~\cite{Kasneci2014} & \textbf{Sippel~\cite{Sippel2014}}  & \textbf{\href{http://www.ti.uni-tuebingen.de/index.php?id=1827\&\&L=1}{ExCuSe}}~\cite{Fuhl2015_ExCuSe}   & \textbf{\href{http://www.ti.uni-tuebingen.de/index.php?id=1827\&\&L=1}{ElSe}}~\cite{Fuhl2016_ElSe} & \textbf{\href{http://www.ti.uni-tuebingen.de/index.php?id=1827\&\&L=1}{Microscope}~\cite{Fuhl2016_Microscope}}  &\textbf{~~~~~~~~LPW~\cite{Tonsen2016_LPW}} & \textbf{RAPD-HD}   \\ \hline


 \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ videos \end{tabular}} &-&40&20  &-&-&- &66 &64 \\ \hline


 %\textbf{FPS} &-&25&25&-&-&-&95 &28 \\ \hline

 \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ frames/images\end{tabular}} &\begin{tabular}[c]{@{}c@{}}3,760 (total)\\  600 (labeled)\end{tabular} &-&-&38,401&55,712&4,263&130,856 & 35,767  \\ \hline


 \textbf{Resolution} &640x480&384x288&384x288&384x288&384x288&512x388&640x480&1,920x1,080\\ \hline

 \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of subjects\end{tabular}}    &2&40&20&17&7 & 2&22 & 22   \\ \hline

 \textbf{\begin{tabular}[c]{@{}c@{}}Acquisition \\ setup\end{tabular}}  &\begin{tabular}[c]{@{}c@{}}head-mounted\\ camera system\end{tabular}&\begin{tabular}[c]{@{}c@{}}head-mounted\\  eye tracker\end{tabular}&\begin{tabular}[c]{@{}c@{}}head-mounted\\  eye tracker\end{tabular}&\begin{tabular}[c]{@{}c@{}}head-mounted\\  eye tracker\end{tabular}&\begin{tabular}[c]{@{}c@{}}head-mounted\\  eye tracker\end{tabular}&microscope & \begin{tabular}[c]{@{}c@{}}head-mounted\\  eye tracker\end{tabular}&headset   \\ \hline


 \textbf{\begin{tabular}[c]{@{}c@{}}Subject \\ activity\end{tabular}}     &-&driving&shopping&\begin{tabular}[c]{@{}c@{}} driving (9)\\ shopping (8)  \end{tabular}&\begin{tabular}[c]{@{}c@{}} driving (5)\\ indoor (2)  \end{tabular}&-&\begin{tabular}[c]{@{}c@{}} staring at a\\ moving target  \end{tabular} &\begin{tabular}[c]{@{}c@{}} staring within\\ a headset  \end{tabular}    \\ \hline

 %\textbf{\begin{tabular}[c]{@{}c@{}}Subject \\ condition\end{tabular}} &-&\begin{tabular}[c]{@{}c@{}} Homonymous \\ visual field \\ defect (10),\\Glaucoma (10) \end{tabular}&\begin{tabular}[c]{@{}c@{}} binocular\\ Glaucoma (10)  \end{tabular}&-&-&-&\begin{tabular}[c]{@{}c@{}} visual \\ impairment (5)  \end{tabular}& \begin{tabular}[c]{@{}c@{}} Glaucoma (),\\ hyphema (),traumatic\\ mydriasis (),\\peripheral RPE\\ atrophy OU (),\\PVD OU  \end{tabular}   \\ \hline
 
 
  \textbf{Metadata} & \begin{tabular}[c]{@{}c@{}}pupil ellipse,  \\ center position\end{tabular}&\begin{tabular}[c]{@{}c@{}}center  \\ position\end{tabular}&\begin{tabular}[c]{@{}c@{}}center  \\ position\end{tabular}&\begin{tabular}[c]{@{}c@{}}center  \\ position\end{tabular}&\begin{tabular}[c]{@{}c@{}}center  \\ position\end{tabular}&\begin{tabular}[c]{@{}c@{}}center  \\ position\end{tabular} &\begin{tabular}[c]{@{}c@{}}pupil ellipse,  \\ center position\end{tabular} & \begin{tabular}[c]{@{}c@{}}swinging flashlight\\ and neutral density \\tests, medical history\end{tabular}    \\ \hline
 
 
 
 
\end{tabular}

\begin{tablenotes}
\item[*] Online sources of the datasets are hyperlinked to the dataset names in the first row of this table.
\end{tablenotes}

\end{threeparttable}
\vspace{-5mm}
\end{table*}



